Informational Puts

We analyze how dynamic information should be provided to uniquely implement the largest equilibrium in binary-action coordination games. The designer offers an informational put: she stays silent if players choose her preferred action, but injects asymmetric and inconclusive public information if they lose faith. There is (i) no multiplicity gap: the largest (partially) implementable equilibrium can be implemented uniquely; and (ii) no commitment gap: the policy is sequentially optimal. Our results have sharp implications for the design of policy in coordination environments.

==> Images/3state_illust_A.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,263); %set diagram left start at 0, and has height of 263

%Shape: Triangle [id:dp6674207630682583] 
\draw   (225,12.3) -- (350,231.3) -- (100,231.3) -- cycle ;
%Straight Lines [id:da8180107702532193] 
\draw [line width=1.5]    (152,140.97) -- (200.5,230.97) ;
%Straight Lines [id:da4667301582328731] 
\draw [line width=1.5]    (200.5,230.97) -- (350,230.3) ;
%Shape: Polygon [id:ds8048729439404196] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=0.2 ] (152,140.97) -- (200.5,230.97) -- (100,231.3) -- cycle ;
%Straight Lines [id:da8382213272039669] 
\draw  [dash pattern={on 3.75pt off 3.75pt on 3.75pt off 3.75pt}]  (225,12.3) -- (185.5,201.47) ;
%Shape: Circle [id:dp27502336851891873] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 200 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 200 }  ,fill opacity=1 ] (196.5,160.25) .. controls (196.5,158.87) and (195.38,157.75) .. (194,157.75) .. controls (192.62,157.75) and (191.5,158.87) .. (191.5,160.25) .. controls (191.5,161.63) and (192.62,162.75) .. (194,162.75) .. controls (195.38,162.75) and (196.5,161.63) .. (196.5,160.25) -- cycle ;
%Straight Lines [id:da2718537110879913] 
\draw  [dash pattern={on 3.75pt off 3.75pt on 3.75pt off 3.75pt}]  (225,12.3) -- (290.5,229.47) ;
%Shape: Circle [id:dp4347994328783493] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 200 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 200 }  ,fill opacity=1 ] (275.5,170.92) .. controls (275.5,169.54) and (274.38,168.42) .. (273,168.42) .. controls (271.62,168.42) and (270.5,169.54) .. (270.5,170.92) .. controls (270.5,172.3) and (271.62,173.42) .. (273,173.42) .. controls (274.38,173.42) and (275.5,172.3) .. (275.5,170.92) -- cycle ;

% Text Node
\draw (168,17.3) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle \Delta ( \Theta )$};
% Text Node
\draw (234,12.3) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle \delta _{1=\theta ^{*}}$};
% Text Node
\draw (350,213.3) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle \delta _{3}$};
% Text Node
\draw (83,212) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle \delta _{2}$};
% Text Node
\draw (129,207) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle \Psi _{LD}( A)$};
% Text Node
\draw (177.37,200.02) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-282.45] [align=left] {$\displaystyle \underbrace{\ \ \ \ \ \ \ \ \ \ \ }_{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }$};
% Text Node
\draw (200,181.3) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {$\displaystyle D\left( \upmu ^{1} ,A\right)$};
% Text Node
\draw (284.76,231.5) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize,rotate=-253.45] [align=left] {$\displaystyle \underbrace{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }_{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }$};
% Text Node
\draw (293,196.98) node [anchor=north west][inner sep=0.75pt]  [font=\tiny] [align=left] {$\displaystyle D\left( \upmu ^{2} ,A\right)$};
% Text Node
\draw (263,239) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle Bd_{\theta ^{*}}$};
% Text Node
\draw (200.52,221.91) node [anchor=north west][inner sep=0.75pt]  [font=\scriptsize] [align=left] {$\displaystyle \underbrace{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ }_{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ } \ \ \ $};


\end{tikzpicture}
